Ducho 2.0: Towards a More Up-to-Date Unified Framework for the Extraction of Multimodal Features in Recommendation

In this work, we introduce Ducho 2.0, the latest stable version of our framework. Differently from Ducho, Ducho 2.0 offers a more personalized user experience with the definition and import of custom extraction models fine-tuned on specific tasks and datasets. Moreover, the new version is capable of extracting and processing features through multimodal-by-design large models. Notably, all these new features are supported by optimized data loading and storing to the local memory. To showcase the capabilities of Ducho 2.0, we demonstrate a complete multimodal recommendation pipeline, from the extraction/processing to the final recommendation. The idea is to provide practitioners and experienced scholars with a ready-to-use tool that, put on top of any multimodal recommendation framework, may permit them to run extensive benchmarking analyses. All materials are accessible at: \url{https://github.com/sisinflab/Ducho}.

==> tables/TEMP_ducho_v2_long_yaml.tex <==
\definecolor{lightgreen}{RGB}{200,255,200}

\begin{listing}[!t]
%\caption{\texttt{config.yml}}
\vspace{-1em}
\begin{minted}[
    frame=lines,
    framerule=0.8pt,
    escapeinside=||,
    fontsize=\footnotesize,
  ]{text}

|\textbf{\textcolor{Black}{dataset\_path}}|: ./my/dataset/path
|\textbf{\textcolor{Black}{gpu list}}|: 0
|\textbf{\textcolor{Mahogany}{visual}}|:
 |\textbf{\textcolor{Black}{items}}|:
  |\textbf{\textcolor{Black}{input\_path}}|:  images
  |\textbf{\textcolor{Black}{output\_path}}|: visual_embeddings
  |\textbf{\textcolor{Black}{model}}|: [
    { |\textbf{model\_name}|: ResNet18, |\textbf{output\_layers}|: avgpool,
      |\textbf{reshape}|: [224, 224], |\textbf{backend}|: torch, |\colorbox{lightgreen}{\textbf{preprocessing}}|: zscore,
      |\colorbox{lightgreen}{\textbf{mean}}|: [0.485, 0.456, 0.406], |\colorbox{lightgreen}{\textbf{std}}|: [0.229, 0.224, 0.225] },
    { |\textbf{model\_name}|: |\colorbox{lightgreen}{"./MyCustomNetWeights.pt"}|, |\textbf{backend}|: torch,
      |\textbf{output\_layers}|: pooler_output, |\colorbox{lightgreen}{\textbf{preprocessing}}|: minmax },
    { |\textbf{model\_name}|: |\colorbox{lightgreen}{"./MyCustomHFModel"}|, |\textbf{backend}|: |\colorbox{lightgreen}{transformers}|,
      |\textbf{output\_layers}|: |[\colorbox{lightgreen}{"MyCustomOutputLayer"}, avgpool]|,
     |\colorbox{lightgreen}{\textbf{image\_processor}}|: "./MyCustomImageProcessor" } ]     
|\textbf{\textcolor{RoyalBlue}{textual}}|:
 |\textbf{\textcolor{Black}{items}}|:
  |\textbf{\textcolor{Black}{input\_path}}|:  descriptions.tsv
  |\textbf{\textcolor{Black}{output\_path}}|: textual_embeddings
  |\textbf{\textcolor{Black}{item\_column}}|: asin
  |\textbf{\textcolor{Black}{text\_column}}|: description
  |\textbf{\textcolor{Black}{model}}|: [
   { |\textbf{model\_name}|: bert-base-uncased, |\textbf{output\_layers}|: pooler_output,
     |\textbf{clear\_text}|: False, |\textbf{backend}|: transformers },
   { |\textbf{model\_name}|: sentence-transformers/all-mpnet-base-v2,  
     |\textbf{clear\_text}|: False, |\textbf{backend}|: sentence_transformers }
   { |\textbf{model\_name}|: |\colorbox{lightgreen}{"./MyCustomHFModel"}|, |\textbf{clear\_text}|: False,
     |\textbf{output\_layers}|: |\colorbox{lightgreen}{"MyCustomOutputLayer"}|, |\textbf{backend}|: transformers, 
    |\colorbox{lightgreen}{\textbf{tokenizer\_name}}|: |"./MyCustomTokenizer"| } ] 
|\colorbox{lightgreen}{\textbf{\textcolor{RoyalPurple}{visual\_textual}}}|:
 |\textbf{\textcolor{Black}{items}}|:
  |\textbf{\textcolor{Black}{input\_path}}|:  { |\textbf{visual}|: images, |\textbf{textual}|: meta.tsv }
  |\textbf{\textcolor{Black}{output\_path}}|: { |\textbf{visual}|: vis_embeddings, |\textbf{textual}|: text_embeddings }
  |\textbf{\textcolor{Black}{item\_column}}|: asin
  |\textbf{\textcolor{Black}{text\_column}}|: description
  |\textbf{\textcolor{Black}{model}}|: [
   { |\textbf{model\_name}|: openai/clip-vit-base-patch16, |\colorbox{lightgreen}{\textbf{fusion}}|: concat, 
     |\textbf{output\_layers}|: 1, |\textbf{backend}|: transformers  } ]
\end{minted}
\caption{An example of a YAML file.}
\label{lst:tempducho_v2_yaml}
\end{listing}

